Benchmark of quantum-inspired heuristic solvers for quadratic unconstrained binary optimization

Recently, inspired by quantum annealing, many solvers specialized for unconstrained binary quadratic programming problems have been developed. For further improvement and application of these solvers, it is important to clarify the differences in their performance for various types of problems. In this study, the performance of four quadratic unconstrained binary optimization problem solvers, namely D-Wave Hybrid Solver Service (HSS), Toshiba Simulated Bifurcation Machine (SBM), Fujitsu DigitalAnnealer (DA), and simulated annealing on a personal computer, was benchmarked. The problems used for benchmarking were instances of real problems in MQLib, instances of the SAT-UNSAT phase transition point of random not-all-equal 3-SAT(NAE 3-SAT), and the Ising spin glass Sherrington-Kirkpatrick (SK) model. Concerning MQLib instances, the HSS performance ranked first; for NAE 3-SAT, DA performance ranked first; and regarding the SK model, SBM performance ranked first. These results may help understand the strengths and weaknesses of these solvers.

==> mqlib_5min_wins.tex <==
\begin{tabular}{l||cccc|cccc|cccc||cccc}\hline
\multicolumn{1}{l||}{} & \multicolumn{4}{c|}{Small} & \multicolumn{4}{c|}{Medium}& \multicolumn{4}{c||}{Large}& \multicolumn{4}{c}{Total}\\ \hline \hline
& HSS & SBM & DA & SA & HSS & SBM & DA & SA & HSS & SBM & DA & SA & HSS & SBM & DA & SA\\\hline
Sparse & 5 & 4 & 2 & 1& 1 & 0 & 2 & 2& 2 & 2 & 1 & 0 & 8 & 6 & 5 & 3\\\hline
Medium & 5 & 3 & 1 & 1& 1 & 1 & 2 & 1& 1 & 1 & 5 & 0 & 7 & 5 & 8 & 2\\\hline
Dense & 4 & 3 & 1 & 0& 3 & 2 & 2 & 1& 0 & 0 & 4 & 1 & 7 & 5 & 7 & 2\\\hline\hline
Total & 14 & 10 & 4 & 2 & 5 & 3 & 6 & 4& 3 & 3 & 10 & 1 & 22 & 16 & 20 & 7\\\hline
\end{tabular}



==> supply.tex <==
The problem instances used in benchmarking is generated on Ubuntu 20.04.3 LTS
\begin{lstlisting}[caption=python code]
import time

def main():
	time.sleep(5)
	print "ok"

#testtest 
if __name__ == "__main__":
	main()

\end{lstlisting}
\begin{lstlisting}[caption=python code]
import numpy as np
import os
import random
import itertools
def random_NAE3SAT(N, M, seed):
    random.seed(a=seed)
    vals = range(1, N+1)
    signs = range(-1, 2, 2)
    randvals = lambda : random.sample(vals, 3)
    randsigns = lambda : random.choices(signs, k=3)
    Jmat = {}
    for i in range(M):
        clause = randvals()
        negs = randsigns()
        #print(clause, negs)
        for pair, sig in zip(itertools.combinations(clause, 2),itertools.combinations(negs, 2)):
            Jmat[pair] = Jmat.get(pair, 0) + np.prod(sig)
    #print(Jmat)
    hvec = {}
    bqm = dimod.BinaryQuadraticModel.from_ising(hvec, Jmat, M)
    return bqm
\end{lstlisting}

\begin{lstlisting}[caption=python code]
import random
rand = lambda : random.gauss(mu, sigma)
  for i in range(N):
            for j in range(i+1,N):
                if rand_dil():
                    Jmat[(i, j)] = rand()/np.sqrt(N)
\end{lstlisting}
